Learning General Inventory Management Policy for Large Supply Chain Network

Inventory management in warehouses directly affects profits made by manufacturers. Particularly, large manufacturers produce a very large variety of products that are handled by a significantly large number of retailers. In such a case, the computational complexity of classical inventory management algorithms is inordinately large. In recent years, learning-based approaches have become popular for addressing such problems. However, previous studies have not been managed systems where both the number of products and retailers are large. This study proposes a reinforcement learning-based warehouse inventory management algorithm that can be used for supply chain systems where both the number of products and retailers are large. To solve the computational problem of handling large systems, we provide a means of approximate simulation of the system in the training phase. Our experiments on both real and artificial data demonstrate that our algorithm with approximated simulation can successfully handle large supply chain networks.

==> nihongo/nihongo_intro.tex <==
大手メーカーのサプライチェーンネットワークは巨大だ。それらのメーカーは、数千ラインナップにもわたる自社製品を、全国各地の数万の店舗の需要を満たすように配送している。その巨大さゆえ、配送計画がわずかでも改善できれば、企業のコスト削減にとっては多大なる貢献になる。だから大手メーカーにとって、商品の配送は重要課題だ。

そのような理由で、サプライチェーンの最適化は古くから研究されてきた問題である。この問題において、サプライチェーンネットワークは、複数の施設 (工場・倉庫・小売店) とそれらの間の配送路でモデル化される。各施設は、より下流の施設にのみ商品を配送する――工場は倉庫あるいは小売店に、倉庫は別の倉庫あるいは小売店に。各配送路に沿って、どの商品を、いつ、どれくらい送るかを決めることで、ネットワークのコストを最小化することが目的となる。

サプライチェーンの最適化には、古典的な○○をはじめとして、○○、○○などのアルゴリズムが知られており[]、小規模なネットワークに対して高性能のアルゴリズムである。近年では商品の需要を時系列データとみなした強化学習に基づく手法が一定の成功を収めている[]。古典的な XX や XX と比べ、強化学習ベースの手法は、季節などの理由による需要量の変動を扱いやすいという点が優れている。とくに Sultana et al. は商品の種類数が多い場合について、実データに対しても高性能なアルゴリズムを開発している。

学習ベースのアプローチは、商品や小売店に対して汎用的な配送戦略を学習する。この主な利点は、学習結果を未知の商品や小売店にも適用できることだ。そして現実において、商品や小売店が未知なのはよくあることだ――メーカーは新製品を開発したり、古い製品の生産を中止したりする。小売店は新たにできたり、逆に閉店したりする。

学習ベースのアプローチの利点はそれだけにとどまらない。Sultana el al. が指摘しているとおり、巨大なネットワーク上での配送最適化には計算量上の問題がある。すなわち、各商品や小売店の配送戦略をひとつずつ最適化するのは、巨大なネットワークでは困難なのだ。

対照的に、学習ベースのアプローチでは、その問題は起こらない。すなわち、汎用的な戦略を一度学習すれば、あとはその戦略をすべての商品や小売店に適用すればよいのだ。たしかに、汎用的な戦略の学習は個別戦略の学習よりも難しい。だがそれでも、系が巨大ならば、前者の方が高速になる。

本研究は、商品の種類数 $P$ と店舗の個数 $R$ の両方が大きいケースに対し、強化学習に基づく倉庫の最適化アルゴリズムを提案する。アルゴリズムへの入力は、単一商品の小売店からの需要履歴をあらわす時系列データである。各時間ステップにおいて、アルゴリズムはその商品を工場へ発注する量を出力する。需要履歴は逐次的に与えられるため、アルゴリズムは未来の需要量を見ることはできない、予測値を知ることはできるが。

複数の商品に対応するため、我々は Sultana et al. の手法に倣う。我々は小売店からの需要のデータや需要予測だけでなく、各商品の情報 (価格や在庫コストなど) をも学習への入力とみなす。そうすることで、学習した配送戦略を、どの商品の在庫管理にも適用できるようになる。

店舗の個数が多い場合の問題は、学習の各ステップでのシミュレーションの計算量が大きいことだ。具体的には、学習の各時間ステップで、全小売店における全商品の配送計画をシミュレートする必要がある。このデータは $O(PR)$ 個にもわたる。巨大な系において、これは無視できないオーバーヘッドである。

この問題を解消するため、われわれは現在シミュレートしている商品以外を近似的に扱うことで、計算量のレベルでシミュレーションを高速化した。この工夫によって、各ステップでのシミュレーションの計算量は $O(R)$ 時間へと削減される。

学習アルゴリズムは PPO アルゴリズムを用いた。われわれはこのアルゴリズムを、実データを入力として性能評価した。データは、Instacart というオンラインショッピングサービスの販売データ [] を適切に加工した、100 商品 100 小売店のものを用いた。

比較対象としては、base-stock policy と呼ばれる古典的な手法を用いた。直観的には、この手法はつねに一定の在庫量を保つことを目標にする。在庫量の目標値をすべての商品に対して決定するために、我々は Optuna を用いたパラメータ最適化を用いた。

我々のアルゴリズムは比較対象よりよい性能を示した。この結果は、われわれの提案する高速化のための近似が、学習に利用するうえではでじゅうぶんに正確であることを示している。




倉庫の在庫管理の難しい点は、施設の在庫量の管理にある。まず、施設の在庫が少なすぎれば、その施設は頻繁に、もしくは恒常的に品切れを起こす。その施設が小売店ならば、しばしば顧客からの需要をさばききれず、あげられるはずだった利益をあげられないことになる。もしその施設が工場や倉庫ならば、下流の倉庫や小売店の注文を満足できず、それらの施設の在庫管理の自由度を下げることになる。

逆に、施設の在庫が多すぎるのも問題だ。在庫は単純に施設の面積を食う。消費期限のある商品の場合、過剰な在庫は在庫の廃棄につながる。型落ちのある商品の価値は、時間とともに目減りする。すなわち、在庫の過剰は、それ自体がコストとみなせる。これらの在庫不足と在庫過剰のトレードオフのバランスを取るのが、サプライチェーンの最適化だとも呼べるだろう。

この問題の解法には、大きく分けて二つのストリームがある。片方は古典的なルールベースのアプローチで、これらは比較的小規模な問題に対して成功を収めている。単一商品に対する最も単純な戦略は base-stock policy だろう。この戦略は、未到着分まで含めた在庫量を常に一定の目的値に保つように発注を行う。目的値の決定のためには、最急降下法に基づくアプローチや、それを微分不可能な目的関数でも動くように拡張した XX アプローチが知られている。また、発注それじたいにかかるコストを加味した base-stock policy の亜種として、$(r,Q)$ policy が知られている。また、そのような目標値を設定せず、需要予測に基づいて各タイムステップで数理計画問題を解くアプローチも存在する[]。

もう一方のアプローチは、学習ベースのアプローチである。2000 年代から研究され始めたこの手法では、需要データを時系列データとみなし、各時間ステップの発注量を強化学習によって決定する。base-stock policy をはじめとする多くのルールベースの手法と異なり、この手法は、需要の季節変化を取り扱うのを得意とする。Sultana et al. は商品に対して汎用的な戦略を学習することで、多商品の場合にも高速かつ効率的に動作するアルゴリズムを設計した。

ほかの研究の方向性として、工場から小売店に至るまでに複数の倉庫を経由する、multi-echelon ネットワーク上でのサプライチェーン最適化が挙げられる。この問題の難しい点は、すなわち下流での需要の細かなブレが、上流での発注量の大変動につながりうる問題――これはブルウィップ効果と呼ばれている――への対処だ。

==> nihongo/nihongo_methodology.tex <==
このセクションでは、商品エージェントたちの戦略を決定するための、われわれのアルゴリズムを説明する。われわれのアルゴリズムは強化学習に基づく。われわれの目的は、どの商品エージェントも汎用的に使えるような在庫管理戦略を学習することである。

商品 $k$ を任意に固定する。まずわれわれは、$k$ 以外すべての商品エージェントの行動を固定することによって、商品エージェント $k$ の在庫管理をマルコフ決定過程とみなす。

状態空間は、前のセクションで導入したすべての変数たちの組合せによって定義される。
行動空間は、日 $t$ には、商品エージェント $k$ が倉庫に商品を発注する量 $order_{t,k}\in \mathbb{R}_{\geq 0}$ である。
遷移関数は、前のセクションで記述した通りである。
報酬関数は、前のセクションで商品エージェント $k$ の gain と記述したものである。

われわれのアルゴリズムでは、単一の強化学習エージェントが、すべての商品エージェント $k$ に対するマルコフ決定過程を用いて学習を行う。具体的には、われわれの強化学習エージェントは、以下を繰り返す: エージェントは $k\in \{1,\dots, P\}$ をランダムに選び、商品エージェント $k$ の $T$ 日ぶんの観測と行動をシミュレーションしながら、方策を更新する。こうして得られた方策は、すべての商品エージェント $k$ に対し、共通に上質な方策となることが期待される。



Remind that われわれの目的は、商品数も小売店数も大きい場合に使える在庫管理アルゴリズムを設計することであった。そのような場合、系全体をシミュレートする計算量は大きい。具体的には、日 $t$ から日 $t+1$ への系の遷移をシミュレートするためには、すべての商品 $k$ とすべての小売店 $i$ に対する、$require_{t,k,i}$ を計算する必要がある。ナイーブには、これには $O(PR)$ 時間がかかる。商品数 $P$ と小売店数 $R$ が両方大きい場合、これは、強化学習のボトルネック部分になる。

そこでわれわれは、その計算量を削減することを考える。訓練を始める前に、われわれはまず、すべての小売店エージェントの行動をシミュレートする。そして、すべての日 $t$, $k$ and $i$ に対し、日 $t$ に小売店 $i$ が倉庫に発注した商品 $k$ の量 $require^*_{t,k,i}$ を記録しておく。このシミュレーションでは、商品エージェントは無限の在庫を持つと仮定する。すなわち、すべての日 $t$ と商品 $k$ と小売店 $i$ に対し、$require^*_{t,k,i}=require_{t,k,i}=ship_{t,k,i}$ となる。Note that, このシミュレーションは訓練段階でのみ行い、評価段階では行わない。

われわれは、この $require^*_{t,k,i}$ たちを用いて、小売店エージェントの行動の近似を計算する。具体的には、任意の $t$, $k$ and $i$ に対し、 $require_{t,k,i}$ の近似値 $require^a_{t,k,i}は、XX で与えられる。
商品エージェント $k$ に関するシミュレーションを行うとき、どの $t$ と $i$ に対しても、$require^a_{t,k,i}$ の値は $O(1)$ 時間で求められる。これは、$require_{t,k,i}$ を求めるのにほかのすべての商品のシミュレーションが必要だったこととは対照的だ。

われわれは、商品エージェントの訓練中、時刻 $t$ の小売店 $i$ の倉庫 $k$ への発注量 $require_{t,k,i}$ の代わりにその近似 $require^a_{t,k,i}$ を用いる。こうすることで、日 $t$ の系を $1$ 日ぶんシミュレートするための計算量は $O(PR)$ 時間から $O(R)$ 時間に削減される。

もちろん、われわれはこの近似がじゅうぶんに正当なものであることを確認せねばならない。その検証のため、われわれは訓練データとは別のデータをもちいて、われわれのアルゴリズムを評価する。評価段階では、われわれは時刻 $t$ の小売店 $i$ の倉庫 $k$ への発注量として、真の値 $require_{t,k,i}$ をそのまま用いる。Note that 評価段階における、$require_{t,k,i}$ の計算時間の大きさは問題にならない、なぜなら、評価段階は、系全体の $T$ 日ぶんのシミュレーションを $1$ 度しか動かさないからである。






訓練アルゴリズムによって現在シミュレートされている商品エージェントを $k$、現在シミュレートされている日を $t$ とする。われわれの機械学習エージェントに与えられる観測は、$3$ つのパートからなる。ひとつめは、商品エージェント $k$ に関する情報である。

これは、$price_k$, $stockcost_k$ and $delay_k$ からなる。

Note that 商品エージェントの添え字 $k$ そのものは、観測に含まれない、未知の商品にも対応できる学習エージェントを作り出すために。
ふたつめは、現在商品エージェント $k$ が持つ商品 $k$ の、工場へと発注はしたがまだ商品エージェント $k$ が受け取っていないぶんまで含めた在庫量 XXX である。
みっつめは、需要予測である。商品エージェントのモデルの節で説明した通りである。

これらの観測は表 $1$ にまとめられている。

==> nihongo/nihongo_model.tex <==
われわれのサプライチェーンネットワークは、$R$ 個の小売店と $P$ 個の商品でモデル化される。各小売店は全 $P$ 商品の在庫を管理する。在庫管理のアルゴリズムの目的は、倉庫が商品を工場へ注文する量と小売店へ発送する量を決定することで、倉庫の在庫をコントロールすることである。われわれは商品の量をキログラム単位で表す。

小売店での需要量は $T$ 日間にわたった時系列データとして与えられる。$t$ 日目の行動を決定する際、在庫管理のアルゴリズムは $t-1$ 日目までの需要量を見ることができる。アルゴリズムは未来の需要量を知ることはできない、需要の予測値を知ることはできるが。

われわれは各小売店にひとつのエージェントを対応付ける。これらのエージェントを、われわれは小売店エージェントと呼ぶ。各小売店エージェントは毎日一回、すべての商品について、倉庫への発注量を決定する。

また、われわれは各商品に対し、倉庫でのその商品の在庫量を管理するエージェントをひとつずつ用意する。これらのエージェントを、われわれは商品エージェントと呼ぶ。
断っておけば、これは倉庫が物理的に複数存在する状況をモデル化しているわけではない。われわれの想定では、倉庫は物理的にはひとつだ――それを管理するエージェントは商品の数だけ存在するが。

小売店エージェントの決定を考慮に入れて、各商品エージェントは毎日一回、対応する商品を各小売店に発送する量を決定する。また、在庫の維持のため、対応する商品を工場へ発注する量を決定する。倉庫が小売店に発送した商品は、特定の日数後に小売店に到着する。到着までにかかる日数は小売店に依存する――これは直感的には、倉庫から小売店へトラックが向かうのにかかる時間をあらわしている。同様に、倉庫が工場へと発注した商品は、特定の日数後に倉庫に到着する。到着までにかかる日数は商品に依存する――これは直感的には、工場が注文を受けて商品を生産し、それを倉庫へと配達するのにかかる時間をあらわしている。

日ごとの各商品エージェントの利得は、ふたつの要素で決定される。ひとつは小売店に発送した商品量である。その日の倉庫の利益は、その量にキログラム当たりの売価を掛けたものとして定式化される。もうひとつは在庫コストであり、それはその日に倉庫に残った在庫量に比例する。各日の商品エージェントの利得は、利益から在庫コストを引いた値である。商品エージェントの総利得は、$T$ 日にわたった利得の合計であり、倉庫の利得は、すべての商品エージェントの利得の合計である。




各商品 $k\in \{1,\dots, P\}$ に対し、われわれはその商品に対応するひとつの商品エージェント $k$ を用意する。各商品エージェント $k$ は、$3$ つの値 $price_k stockcost_k\in \mathbb{R}^{\geq 0}$ と $delay_k\in mathbb{Z}^{>0}$ を持っている。

これらの値は、商品 $k$ に関する情報をあらわす。具体的には、$price_k$ は $1$ キログラム当たりの商品 $k$ の売価をあらわす。$stockcost_k$ は、各日のおわりにに倉庫に残った商品 $k$ の在庫 $1$ キログラムあたりにかかる、在庫コストをあらわす。$delay_k$ は、商品エージェントが商品 $k$ を工場へと発注してから倉庫に到着するまでの日数をあらわす。われわれは、商品はいくらでも細かく分割して輸送できると仮定する――すなわち、倉庫が工場に発注する商品の量や、倉庫が小売店に発送する商品の量は、在庫が足りている限りにおいて任意の実数値を取りうる。

各日 $t$ の商品エージェント $k$ の行動は以下の通りである。まずエージェントは、時刻 $t-delay_k$ に工場へと発注した商品を受け取る。また、時刻 $t$ における、商品 $k$ を小売店エージェントたちから発注された量を確認する。以上のふたつの情報から、商品エージェント $k$ は、時刻 $t$ に商品 $k$ を工場に発注する量 $order_{t,k}\in \mathbb{R}^{\geq 0}$ を決定する。われわれは、工場は無限の生産能力を持つと仮定する――すなわち、値 $order_{t,k}$ は任意の非負実数値を取りうる。また、各小売店 $i\in \{1,\dots, R\}$ に対し、時刻 $t$ に商品 $k$ を小売店 $i$ に発送する量 $sell_{t,k,i}\in \mathbb{R}^{\geq 0}$ を決定する。

時刻 $t$ に倉庫に残った商品 $k$ の在庫量を $stock_{t,k}$ で表すことにすれば、日 $t$ における $stock_{t,k}$ の更新式は以下のとおりである。


また、これらの値を用いれば、時刻 $t$ における商品エージェント $k$ の利得は以下のように書き表せる。


商品エージェントが商品を工場へ発注する量を管理することを考えるのに集中するため、われわれは商品エージェントが小売店に商品を発送するための戦略を固定する。直観的には、われわれの戦略は、「来た注文にはこたえられる限りこたえる」である。商品エージェントの利得を最大化する目的では、これは正しい戦略である。キログラム当たりの商品の価格は日によって変わらず、余剰の在庫を残してもただ在庫コストがかさむだけであることが、この理由である。


小売店エージェントたちが商品 $k$ を倉庫に発注したとき、われわれの設計する商品エージェント $k$ は、倉庫に商品 $k$ の在庫がある限りは発送する。すなわち、仮に時刻 $t$ における小売店エージェント $i$ の商品 $k$ の発注量を $demand_{t,k,i}$ とすれば、XX である。

$sell_{t,k}=\sum_{i\in \{1,\dots, R\}}demand_{t,k,i}$ のときは、日 $t$ に、商品エージェント $k$ はすべての小売店エージェントの注文にこたえられるだけの在庫を持っていることをあらわす。その場合、日 $t$ に、商品エージェント $k$ は各小売店エージェント $i$ に、ちょうど $demand_{t,k,i}$ だけの商品を発送する。

逆にそうでないときは、日 $t$ の商品エージェント $k$ が持つ在庫は、すべての小売店エージェントの注文にこたえるには足りないことをあらわす。その場合、われわれの設計する商品エージェント $k$ は、日 $t$ に持っている在庫すべてを、各小売店の注文量と各小売店への発送量が比例するように発送することにする。厳密には、商品エージェント $k$ が小売店エージェント $i$ に日 $t$ に発送する商品 $k$ の量は、







==> nihongo/nihongo_retail_model.tex <==
各小売店 $i\in \{1,\dots, R\}$ に対し、われわれはその小売店に対応するひとつの小売店エージェント $i$ を用意する。各小売店エージェント $i$ は、$2$ つの値 $trucksize_i\in \mathbb{R}^{\geq 0}$ と$delay_i\in mathbb{Z}^{>0}$ を持っている。

これらの値は、小売店 $i$ に関する情報をあらわす。具体的には、$trucksize_i$ は、倉庫から小売店 $i$ へと向かうトラックに積載できる、商品の量の最大値をあらわす。トラックは、合計の重量が $trucksize_i$ キログラムを超えない範囲で、すべての種類の商品を任意の組合せで、任意の非負実数量だけ輸送することができる。
$delay_i$ は、小売店が倉庫に商品を注文してから、その商品を積んだトラックが小売店に到着するまでにかかる日数をあらわす。

各日 $t$ における小売店エージェント $i$ の行動は以下のとおりである。まずエージェントは、各商品 $k$ に対し、日 $t-delay_i$ に倉庫が小売店 $i$ へと発送した商品を受け取る。Note that, 小売店エージェントが日 $t$ に受けとる商品の量は、日 $t-delay_i$ に倉庫へと発注した商品の量とは異なるかもしれない。このような事態は、日 $t-delay_i$ の時点で倉庫にじゅうぶんな在庫量がなかった場合に起こりうる。Note that, これは、小売店エージェントに固有の問題だ。工場は無限の在庫を持つので、商品エージェントが工場に発注した商品を受け取るときは、似た問題は起こらない。

その後、小売店エージェント $i$ は、すべての商品 $k$ に対し、日 $t$ に小売店 $i$ が倉庫へと発注する商品 $k$ の量 $request_{t,k,i}$ を決定する。そののち、小売店エージェントは客に商品を売る。日 $t$ に小売店 $i$ が客に売却した商品 $k$ の量を $sales_{t,k,i}$ キログラムとする。

日 $t$ における小売店 $i$ の商品 $k$ の在庫量を $stock_{t,k,i}$ とすれば、日 $t$ における $stock_{t,k,i}$ の更新式は以下のとおりである。


われわれは、小売店エージェントが客に商品を販売するための戦略を固定する。直観的には、われわれの戦略は、「需要をできるだけ満たす」である。厳密には、日 $t$ における小売店 $i$ における商品 $k$ の客からの需要量を $demand_{t,k,i}$ とすれば、$sales_{t,k,i}$ は、 X で表される。


再度言うが、われわれの考えるシチュエーションでは、商品エージェントたちは小売店エージェントたちの行動をコントロールできない。そのため、われわれは小売店エージェントたちの行動を最適化するのではなく、戦略を固定する。同じ理由で、われわれは店舗エージェントたちの利得を厳密には定義しない。

われわれの設計する小売店エージェントの戦略を紹介する前に、われわれが小売店のシチュエーションがどうあると考えているかを説明しよう。
Note that, モデルの数学的詳細を理解するためだけなら、たしかにこの説明を知る必要はない。そのかわりに、このシチュエーションの説明はむしろ、小売店エージェントの戦略の妥当性を理解する助けになる。

われわれの想定するシチュエーションにおいて、小売店エージェントの利得は、商品を客に販売することによる利益と、商品の在庫を持つことのコスト、また商品を倉庫から輸送してくるために必要なコストによって決定される。
まず、店舗の利益は、商品を客に売却した量 $sales_{t,k,i}$ たちによって決定される。具体的には、小売店エージェント $i$ の利益は、$sales_{t,k,i}$ の、各日 $t$ と各商品 $k$ にわたった非負結合として書き表される。
同様に、小売店エージェント $i$ の在庫コストは、各日のおわりに売れ残った商品の在庫量 $stock_{t,k,i}$ の、各日 $t$ と各商品 $k$ にわたった非負結合として書き表される。

最後に、商品を倉庫から輸送してくるために必要なコストを設計する。われわれが重要視するのは、商品の輸送のために倉庫から小売店へとトラックを動かすという行為じたいにかかるコストである。このコストは、その日に輸送される商品の量が $0$ かそうでないかにのみ依存する。具体的には、日 $t$ と小売店 $i$ に対し、もしある商品 $k$ が存在して $ship_{t,k,i}>0$ なら、その日、その小売店には、一定のコストがかかる。

これは次のような事実を表現している、 トータルで同じ量の商品を輸送するのなら、少しずつ小分けにして輸送するよりも、一度にたくさん輸送した方が効率的だ。特にこの項は、このような小売店にとって重要である、われわれが在庫を管理する倉庫から商品を輸送してくる量が比較的少なく、一日分に適した発注量だけでは一台のトラックをいっぱいにできないような。





%われわれの戦略は、古典的な $(r,Q)$ reorder policy [] を、複数の商品がある場合に拡張したものである。なお、$(r,Q)$ reorder policy は、商品数がひとつで、倉庫から小売店へとトラックを動かすという行為じたいにコストがかかる場合に、古典的によく用いられる手法である。


それでは、われわれの設計する小売店エージェントの戦略を紹介する。各小売店エージェント $i$ は、各商品 $k$ に対し、実数値 $basestock_{k,i}\in \mathbb{R}_{>0}$ を持っている。基本的には、古典的な base-stock policy []のように、小売店エージェントは、各商品の未到着分まで含めた在庫量を一定値に保つように行動しようとする。具体的には、小売店エージェント $i$ が 日 $t$ に商品エージェント $k$ に発注しようとする商品 $k$ の量は、XXX で表される。

だがこの戦略に従えば、いちどに少量の商品だけを輸送することが、頻繁に発生することになってしまう。じっさい、簡単にわかることだが、小売店でゼロでない量の商品が売れるたびに輸送が発生してしまう。この問題を避けるため、われわれは戦略を少し修正し、日 $t$ に小売店 $i$ が発注しようとする商品の合計量がトラックの積載容量を超えたときにのみ発注が行われるようにする。フォーマルには、小売店エージェント $i$ が発注を行うのは、YYY が満たされるときだけである。また、そのときに発注する商品の量は、トラックの積載容量ちょうどに収まるように正規化される。具体的には、上の条件が満たされているとき、小売店エージェント $i$ が日 $t$ に倉庫に発注する商品 $k$ の量は、ZZZ である。

この工夫により、もし倉庫がつねに十分な在庫を持っていれば、倉庫から小売店へ商品を輸送するトラックはつねにいっぱいであることになる。


